Efficient Dynamic Mesh Refinement Technique for Simulation of HPM Breakdown induced Plasma Pattern Formation

Numerical simulation of the complex plasma dynamics associated with high power, high frequency microwave breakdown at high pressures, leading to the formation of filamentary plasma structures such as self-organized plasma arrays, is a computationally challenging problem. The widely used 2D EM-plasma fluid model, which accurately captures the experimental observations, requires a run-time of several days to months to simulate standard problems due to stringent numerical requirements in terms of cell size and time step. In this paper, we present a self-aware mesh refinement algorithm which uses a coarse mesh and a fine mesh that dynamically expands based on the plasma profile topology to resolve the sharp gradients in E-fields and plasma density in the breakdown region. The dynamic mesh refinement (DMR) technique is explained in details and its performance has been evaluated using a standard benchmark microwave breakdown problem. We observe a speedup of 8 (of the order of $O(r^{3})$, when refinement factor ($r$) is 2) compared to a traditional single uniform fine mesh based simulation. The technique is scalable and performs better when problem size increases. We also present a comprehensive spatio-temporal visual analysis to explain the complex physics of HPM breakdown, leading to self-organized plasma filamentation.

==> arxiv-DMR_Paper_IEEEPlasmaScience(Final) (Copy)/introduction.tex <==
\section{Introduction} \label{sec:intro}

High power microwave (HPM) breakdown have been studied theoretically as well as experimentally since the 1950s for a wide variety of applications such as aerodynamic flow control, combustion,  precision radar systems, energy deposition in super- and hyper-sonic gas dynamic flows, beamed energy propulsion, deep-space communications applications, electromagnetic warfare, ultra-wideband (UWB) HPM transmission, to name a few ~\cite{ ADMacdonald1966,Khodataev2008,Nusinovich1997,Saifutdinov2019,MFukunari2018,JBenfordHPMdeepspapp2008,HPMwarfare2000,HPMeffectUWBtransmission2010}. 
However, only recently, detailed experimental investigations of the plasma dynamics during breakdown have been possible with the use of sophisticated high-speed cameras \cite{Hidaka2009,AMCook2011,Schaub2016,Fukunari2019,Oda2020}. Particularly, in the past few years, several experiments using millimeter and sub-millimeter wave irradiation (100s of GHz) at high pressures (ten to hundreds of Torr) have been carried out~\cite{Khodataev2008,Hidaka2008,Hidaka2009,Fukunari2019,Schaub2016,Aleksandrov2006,Oda2020,Yoda2006,AMCook2011,PBulat2021}. Different types of gas discharges have been reported experimentally such as streamer, overcritical, subcritical, volumetric and attached to an initiator~\cite{Khodataev2008,Aleksandrov2006,PBulat2021}. To completely understand the properties of each type of discharge, it is crucial to further improve our current understanding of the electromagnetic (EM) wave-plasma interaction, plasma formation, the subsequent energy exchange between wave and plasma, and
afterwards between the gas and the plasma. 
The modeling and simulation of the interaction of high power high frequency EM wave with air/gas is a computationally challenging problem \cite{BChaudhury2010,Konstantinos-2015,Saifutdinov2021,HAMIAZ2020,BCHAUDHURY2018,Kourtzanidis20143DHPM}. 
Different semi-analytical models and computational techniques have been used to study this problem~\cite{NamVerboncoeur2009,BChaudhury2010,BChaudhuryPRL2010,Nakamura2018,Saifutdinov2021,BCHAUDHURY2018,Konstantinos-2015,Kourtzanidis20143DHPM,Yan2019DGTDmesh, VGBrovkin2020,Ref2Wang2020,Bhaskarieee,HAMIAZ2020,Ref3Zhao2011}. \\
\indent
Recent experiments \cite{Hidaka2008,Hidaka2009,Aleksandrov2006, AMCook2011, Khodataev2008,Schaub2016,Yoda2006,Oda2020,Fukunari2019,MFukunari2018,PBulat2021} reveal the formation of self-organized plasma structures, either fish-bone like filaments (in overcritical), or, comb-shaped and branching (in sub-critical), that occur during air breakdown from focused (MW/cm$^{2}$), or, non-focused (kW/cm$^{-2}$) high-frequency microwave under atmospheric pressure, respectively. The plasma structures propagate towards the microwave source. The filaments elongate in the direction of the microwave electric field \cite{BChaudhury2010, Konstantinos-2015}.
The high-density plasma filaments enhance the scattered EM field at the anti-node of standing waves that result from continuous ionization diffusion mechanism and sustain the self-organized plasma pattern formation \cite{BChaudhury2010}. This problem has been used as a benchmark problem by several researchers to perform new investigations or validating the computational techniques \cite{Kourtzanidis20143DHPM,Konstantinos-2015,Semenov2015,MTakahashietal2017,Takahashi-2019,Yan2019DGTDmesh,HAMIAZ2020,Pratik2020}.\\
\indent
Accurate 2D simulations of HPM breakdown experiments mentioned above have been performed using the well established fluid model involving the coupling of Maxwell's equations and plasma continuity equation \cite{BChaudhury2010,BCHAUDHURY2018,QZHAO2011,Ref2Wang2020,Konstantinos-2015}.
It is a complex multi-physics multi-scale model due to the presence of different space and time scales \cite{Yan2019DGTDmesh, BCHAUDHURY2018} which needs to be resolved accurately. Most of the previous works \cite{Bhaskarieee,BChaudhury2010,BCHAUDHURY2018,BChaudhury2011,QZHAO2011,Konstantinos-2015,Kourtzanidis20143DHPM,Takahashi-2019,Nakamura2018,Pratik2020,HPMeffectUWBtransmission2010,Ref3Zhao2011,HAMIAZ2020} used finite difference time domain (FDTD) method in the Maxwell-plasma fluid model based simulations.
Though the simulations quite well reproduce the experimental observations but at the cost of high computation, therefore most of the past 2D numerical investigations using the fluid model have been carried out till hundreds of nanoseconds.
The excessive computational cost is due to stringent restrictions on the grid spacing and time steps \cite{BChaudhury2010,BCHAUDHURY2018,HAMIAZ2020,Konstantinos-2015}. Therefore, it is challenging to simulate large problem sizes over longer timescales (tens of microseconds) using homogeneous mesh having the finest resolution of grid size to capture the gradients in plasma density and the secondary E-field that originates from it. 
Simulation of this complex phenomenon at longer timescales will further help to understand the underlying physics for various applications in microwave rockets \cite{Takahashi-2019, MFukunari2018, Masayuki2017tf}, aerospace research \cite{Khodataev2008,DKnight2009,BCHAUDHURY2018,PBulat2021}, high-speed combustion \cite{JBMichael-2010}, safe operation of high power microwave devices ~\cite{Ref2Wang2020} etc.\\
\indent
Recently, advanced parallelization strategies for emerging many-core architectures have been proposed which significantly reduces the simulation-time, but this requires sophisticated computing facilities~\cite{BCHAUDHURY2018}.
To address the computational challenges associated with the 2D FDTD based EM-plasma fluid model for HPM breakdown, alternative numerical techniques have been developed for both structured meshes \cite{Konstantinos-2015} and unstructured meshes \cite{Yan2019DGTDmesh}. Though, the techniques are capable to balance the trade-off between accuracy and computational cost but requires complex mathematical formulation, proper choice of higher order basis functions and modification of the existing model. Recently, a static mesh refinement (MR) technique for the well established FDTD based fluid model has been presented for studying evolving plasma dynamics \cite{Pratik2020}.
Although, the static MR based technique is accurate and relatively fast compared to single uniform fine mesh, but overall performance is restricted by the size of the fixed preset refined mesh that restricts bigger and longer simulation. Therefore,  a self-aware dynamic mesh refinement (DMR) technique that generates fine mesh on demand based on the plasma evolution is proposed in this paper
The key contributions of this paper are as follows:
\begin{itemize}   
    \item Development and implementation of DMR technique for Maxwell-Plasma fluid model for investigating complex plasma dynamics during HPM breakdown.
    \item Validation and performance analysis of the proposed DMR technique against published results.
    \item To understand and visualize the plasma pattern formation and its spatio-temporal evolution under real experimental conditions using the DMR based code.
\end{itemize}

The remainder of the paper is organized as follows: Section II provides a brief introduction of the physical model, its numerical implementation and the computational challenges associated with a benchmark simulation. In section III, we discuss the theory and implementation of the Dynamic Mesh refinement technique. In Section IV, we report about the accuracy and efficiency of the proposed DMR technique, and subsequently we use our simulation results to provide a detailed spatio-temporal analysis of the complex plasma dynamics during HPM breakdown followed by conclusion in section V.


==> introduction.tex <==
\section{Introduction} \label{sec:intro}

High power microwave (HPM) breakdown have been studied theoretically as well as experimentally since the 1950s for a wide variety of applications such as aerodynamic flow control, combustion,  precision radar systems, energy deposition in super- and hyper-sonic gas dynamic flows, beamed energy propulsion, deep-space communications applications, electromagnetic warfare, ultra-wideband (UWB) HPM transmission, to name a few ~\cite{ ADMacdonald1966,Khodataev2008,Nusinovich1997,Saifutdinov2019,MFukunari2018,JBenfordHPMdeepspapp2008,HPMwarfare2000,HPMeffectUWBtransmission2010}. 
However, only recently, detailed experimental investigations of the plasma dynamics during breakdown have been possible with the use of sophisticated high-speed cameras \cite{Hidaka2009,AMCook2011,Schaub2016,Fukunari2019,Oda2020}. Particularly, in the past few years, several experiments using millimeter and sub-millimeter wave irradiation (100s of GHz) at high pressures (ten to hundreds of Torr) have been carried out~\cite{Khodataev2008,Hidaka2008,Hidaka2009,Fukunari2019,Schaub2016,Aleksandrov2006,Oda2020,Yoda2006,AMCook2011,PBulat2021}. Different types of gas discharges have been reported experimentally such as streamer, overcritical, subcritical, volumetric and attached to an initiator~\cite{Khodataev2008,Aleksandrov2006,PBulat2021}. To completely understand the properties of each type of discharge, it is crucial to further improve our current understanding of the electromagnetic (EM) wave-plasma interaction, plasma formation, the subsequent energy exchange between wave and plasma, and
afterwards between the gas and the plasma. 
The modeling and simulation of the interaction of high power high frequency EM wave with air/gas is a computationally challenging problem \cite{BChaudhury2010,Konstantinos-2015,Saifutdinov2021,HAMIAZ2020,BCHAUDHURY2018,Kourtzanidis20143DHPM}. 
Different semi-analytical models and computational techniques have been used to study this problem~\cite{NamVerboncoeur2009,BChaudhury2010,BChaudhuryPRL2010,Nakamura2018,Saifutdinov2021,BCHAUDHURY2018,Konstantinos-2015,Kourtzanidis20143DHPM,Yan2019DGTDmesh, VGBrovkin2020,Ref2Wang2020,Bhaskarieee,HAMIAZ2020,Ref3Zhao2011}. \\
\indent
Recent experiments \cite{Hidaka2008,Hidaka2009,Aleksandrov2006, AMCook2011, Khodataev2008,Schaub2016,Yoda2006,Oda2020,Fukunari2019,MFukunari2018,PBulat2021} reveal the formation of self-organized plasma structures, either fish-bone like filaments (in overcritical), or, comb-shaped and branching (in sub-critical), that occur during air breakdown from focused (MW/cm$^{2}$), or, non-focused (kW/cm$^{-2}$) high-frequency microwave under atmospheric pressure, respectively. The plasma structures propagate towards the microwave source. The filaments elongate in the direction of the microwave electric field \cite{BChaudhury2010, Konstantinos-2015}.
The high-density plasma filaments enhance the scattered EM field at the anti-node of standing waves that result from continuous ionization diffusion mechanism and sustain the self-organized plasma pattern formation \cite{BChaudhury2010}. This problem has been used as a benchmark problem by several researchers to perform new investigations or validating the computational techniques \cite{Kourtzanidis20143DHPM,Konstantinos-2015,Semenov2015,MTakahashietal2017,Takahashi-2019,Yan2019DGTDmesh,HAMIAZ2020,Pratik2020}.\\
\indent
Accurate 2D simulations of HPM breakdown experiments mentioned above have been performed using the well established fluid model involving the coupling of Maxwell's equations and plasma continuity equation \cite{BChaudhury2010,BCHAUDHURY2018,QZHAO2011,Ref2Wang2020,Konstantinos-2015}.
It is a complex multi-physics multi-scale model due to the presence of different space and time scales \cite{Yan2019DGTDmesh, BCHAUDHURY2018} which needs to be resolved accurately. Most of the previous works \cite{Bhaskarieee,BChaudhury2010,BCHAUDHURY2018,BChaudhury2011,QZHAO2011,Konstantinos-2015,Kourtzanidis20143DHPM,Takahashi-2019,Nakamura2018,Pratik2020,HPMeffectUWBtransmission2010,Ref3Zhao2011,HAMIAZ2020} used finite difference time domain (FDTD) method in the Maxwell-plasma fluid model based simulations.
Though the simulations quite well reproduce the experimental observations but at the cost of high computation, therefore most of the past 2D numerical investigations using the fluid model have been carried out till hundreds of nanoseconds.
The excessive computational cost is due to stringent restrictions on the grid spacing and time steps \cite{BChaudhury2010,BCHAUDHURY2018,HAMIAZ2020,Konstantinos-2015}. Therefore, it is challenging to simulate large problem sizes over longer timescales (tens of microseconds) using homogeneous mesh having the finest resolution of grid size to capture the gradients in plasma density and the secondary E-field that originates from it. 
Simulation of this complex phenomenon at longer timescales will further help to understand the underlying physics for various applications in microwave rockets \cite{Takahashi-2019, MFukunari2018, Masayuki2017tf}, aerospace research \cite{Khodataev2008,DKnight2009,BCHAUDHURY2018,PBulat2021}, high-speed combustion \cite{JBMichael-2010}, safe operation of high power microwave devices ~\cite{Ref2Wang2020} etc.\\
\indent
Recently, advanced parallelization strategies for emerging many-core architectures have been proposed which significantly reduces the simulation-time, but this requires sophisticated computing facilities~\cite{BCHAUDHURY2018}.
To address the computational challenges associated with the 2D FDTD based EM-plasma fluid model for HPM breakdown, alternative numerical techniques have been developed for both structured meshes \cite{Konstantinos-2015} and unstructured meshes \cite{Yan2019DGTDmesh}. Though, the techniques are capable to balance the trade-off between accuracy and computational cost but requires complex mathematical formulation, proper choice of higher order basis functions and modification of the existing model. Recently, a static mesh refinement (MR) technique for the well established FDTD based fluid model has been presented for studying evolving plasma dynamics \cite{Pratik2020}.
Although, the static MR based technique is accurate and relatively fast compared to single uniform fine mesh, but overall performance is restricted by the size of the fixed preset refined mesh that restricts bigger and longer simulation. Therefore,  a self-aware dynamic mesh refinement (DMR) technique that generates fine mesh on demand based on the plasma evolution is proposed in this paper
The key contributions of this paper are as follows:
\begin{itemize}   
    \item Development and implementation of DMR technique for Maxwell-Plasma fluid model for investigating complex plasma dynamics during HPM breakdown.
    \item Validation and performance analysis of the proposed DMR technique against published results.
    \item To understand and visualize the plasma pattern formation and its spatio-temporal evolution under real experimental conditions using the DMR based code.
\end{itemize}

The remainder of the paper is organized as follows: Section II provides a brief introduction of the physical model, its numerical implementation and the computational challenges associated with a benchmark simulation. In section III, we discuss the theory and implementation of the Dynamic Mesh refinement technique. In Section IV, we report about the accuracy and efficiency of the proposed DMR technique, and subsequently we use our simulation results to provide a detailed spatio-temporal analysis of the complex plasma dynamics during HPM breakdown followed by conclusion in section V.

